Automatic Layout Generation with Applications in Machine Learning Engine Evaluation

Machine learning-based lithography hotspot detection has been deeply studied recently, from varies feature extraction techniques to efficient learning models. It has been observed that such machine learning-based frameworks are providing satisfactory metal layer hotspot prediction results on known public metal layer benchmarks. In this work, we seek to evaluate how these machine learning-based hotspot detectors generalize to complicated patterns. We first introduce a automatic layout generation tool that can synthesize varies layout patterns given a set of design rules. The tool currently supports both metal layer and via layer generation. As a case study, we conduct hotspot detection on the generated via layer layouts with representative machine learning-based hotspot detectors, which shows that continuous study on model robustness and generality is necessary to prototype and integrate the learning engines in DFM flows. The source code of the layout generation tool will be available at https://github. com/phdyang007/layout-generation.

==> acm-setting.tex <==
% =============================================================
%         Setting for ACM 2017 format
%
%   Author      : Bei Yu
%   Last Update : 04/2018
% =============================================================

\settopmatter{printacmref=false}          % no ACM Reference Format
\fancyhead{}                              % no header

% ==== page margin settings
\geometry{twoside=true, head=13pt,
	paperwidth=8.5in, paperheight=11in,
	includeheadfoot, columnsep=2pc,
	top=57pt, bottom=73pt, inner=54pt, outer=54pt,
	marginparwidth=2pc,heightrounded
}%
\iffalse
\textfloatsep          = 10pt plus 1pt minus 7pt           % set space between figure and text
\floatsep              =  4pt plus 1pt minus 7pt
\fi
%\intextsep             = 0pt plus 1pt minus 7pt           % set space above and below the texts
%\dbltextfloatsep       = 0pt plus 1pt minus 7pt
%\dblfloatsep           = 0pt plus 1pt minus 7pt
%\abovedisplayskip      = 0pt plus 1pt minus 7pt           % set space around equations
%\belowdisplayskip      = 0pt plus 1pt minus 7pt
%\abovedisplayshortskip = 0pt plus 1pt minus 7pt
%\belowdisplayshortskip = 0pt plus 1pt minus 7pt

% ==== Packages
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{comment}
\usepackage[subrefformat=parens,labelformat=parens]{subfig}
\captionsetup[subfigure]{labelformat=simple}               % avoid "double brackets" in sub-figure caption
\renewcommand\thesubfigure{(\alph{subfigure})}             % "Fig.~1b"-->"Fig.1(b)"
\usepackage{bm}
\usepackage{multirow}
\usepackage{threeparttable,booktabs}
\usepackage{blkarray}
\usepackage{tikz}
\usepackage{balance}
\usepackage{courier}                                       % courier font, used in \texttt
\usepackage{cleveref}                                      % smart citation
\usepackage[mathcal]{eucal}
\usepackage[]{algpseudocode}                               % algorithm package
%\usepackage[noend]{algpseudocode}
\algrenewcommand\textproc{\texttt}
\makeatletter\let\float@addtolists\relax\makeatother
\usepackage{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:} }       % Use Input in the format of Algorithm
\renewcommand{\algorithmicensure} {\textbf{Output:}}       % Use Output in the format of Algorithm
\usepackage{filecontents}                                  % support to pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
%\usepackage{rotating} 
\usepackage[figuresright]{rotating}
\usepackage{flexisym}

% ==== Local new commands
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\DeclareMathOperator*{\argmin}{argmin}

\theoremstyle{plain}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}

\theoremstyle{definition}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{myproblem}{\textbf{Problem}}



% ==== spacing control on caption
\usepackage[skip=1pt]{caption}            % set space between figure and caption
\setlength{\belowcaptionskip}{-1.0mm}
\captionsetup[table]{aboveskip=5pt}       % reduce space around table caption
\captionsetup[table]{belowskip=2pt}

